SemGeoMo: Dynamic Contextual Human Motion Generation with Semantic and Geometric Guidance

Generating reasonable and high-quality human interactive motions in a given dynamic environment is crucial for understanding, modeling, transferring, and applying human behaviors to both virtual and physical robots. In this paper, we introduce an effective method, SemGeoMo, for dynamic contextual human motion generation, which fully leverages the text-affordance-joint multi-level semantic and geometric guidance in the generation process, improving the semantic rationality and geometric correctness of generative motions. Our method achieves state-of-the-art performance on three datasets and demonstrates superior generalization capability for diverse interaction scenarios. The project page and code can be found at https://4dvlab.github.io/project_page/semgeomo/.

==> rebuttal.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}
% \usepackage[rebuttal]{cvpr}

% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}
% \usepackage{colortbl}  %彩色表格需要加载的宏包
% \usepackage{xcolor}


% % Import additional packages in the preamble file, before hyperref
% \input{preamble}

% % If you comment hyperref and then uncomment it, you should delete
% % egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% % run, let it finish, and you should be clear).
% \definecolor{cvprblue}{rgb}{0.21,0.49,0.74}

% \usepackage[pagebackref,breaklinks,colorlinks,allcolors=cvprblue]{hyperref}
% \newcommand{\textred}{\textcolor[rgb]{1.0,0.0,0.0}}
% \newcommand{\notes}{\textcolor[rgb]{0.6,0.6,0.6}}
% \newcommand{\reply}{\textcolor[rgb]{0.9,0.6,0}}
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}
% \usepackage{ulem}
% \usepackage{wrapfig}
% \definecolor{dgreen}{rgb}{0.0,0.6,0.0}
% \newcommand{\cmark}{\textcolor{dgreen}{\text{\ding{51}}}}%

% % If you wish to avoid re-using figure, table, and equation numbers from
% % the main paper, please uncomment the following and change the numbers
% % appropriately.
% %\setcounter{figure}{2}
% %\setcounter{table}{1}
% %\setcounter{equation}{2}

% % If you wish to avoid re-using reference numbers from the main paper,
% % please uncomment the following and change the counter value to the
% % number of references you have in the main paper (here, 100).
% %\makeatletter
% %\apptocmd{\thebibliography}{\global\c@NAT@ctr 100\relax}{}{}
% %\makeatother

% %%%%%%%%% PAPER ID  - PLEASE UPDATE
% \def\paperID{8324} % *** Enter the Paper ID here
% \def\confName{CVPR}
% \def\confYear{2025}

% \begin{document}

% %%%%%%%%% TITLE - PLEASE UPDATE
% \title{\LaTeX\ Guidelines for Author Response}  % **** Enter the paper title here

% % \maketitle
% \thispagestyle{empty}
% \appendix

% \iffalse
% \begin{table*}[h]
% \vspace{-1ex}
% % \caption{Ablation study on joint constraint control.}
% \resizebox{\linewidth}{!}{ 
% \centering
% \begin{tabular}{c|cccccccccccc}
% \hline
% method & HandJPE$\downarrow$                                & MPJPE$\downarrow$                               & $C_{prec} \uparrow$                       & $C_{rec}\uparrow$                       & $C_{acc}\uparrow$ & $C\% \uparrow$    & F1$\uparrow$   & FID$\downarrow$ & R-score$\uparrow$   & Diversity$\uparrow$ & FS$\downarrow$  \\ \hline
% AffordMotion                        &    98.66        &   25.34    & 0.45           & 0.14           &    0.31          &    0.13 &  0.16  &  4.71   &  0.45  & 8.15 & 0.43  \\ \hline
% AffordMotion-Loss            &  53.72                           & 21.60                               & 0.69                         & 0.26                            & 0.45       & 0.23    & 0.36 &   4.13  &    0.47     &8.25& 0.65      \\ \hline
% Ours (w/o Loss)                      &  84.29          &   22.89    &   0.61    &  0.20   & 0.38           &        0.21      &   0.25  & \textbf{0.89}   &  \textbf{0.67}    & 10.05 & \textbf{0.38}   \\ \hline
% Ours                                 &   \textbf{27.84}         &   \textbf{16.62}    &  \textbf{0.84}          &     \textbf{0.74}       &       \textbf{0.85}       &   \textbf{0.66}  &  \textbf{0.77}  &  1.17   &   0.66  &  \textbf{10.15}  &  0.57  \\ \hline
% \end{tabular}
% }
% \label{tab:rebuttal-loss}
% \vspace{-2ex}
% \end{table*}
% \fi



% We express our gratitude to all reviewers for \textbf{recognizing our contribution, the effectiveness of our method, and solid experiment (\textcolor{red}{mWgN}, \textcolor[rgb]{0.55, 0.8, 0.25}{jgcn}, \textcolor{blue}{WDaT})}. Hope the following replies could clarify your concerns.

 
% \noindent\textcolor{red}{\textbf{(mWgN)}}
% \reply{\textbf{\uline{Differences between ours and AffordMotion}}} 
% \textbf{(1) Improved Affordance Map Quality:} In the first stage, our method incorporates mutual information exchange between joint and affordance maps, improving affordance map quality, with the map similarity score increasing from 0.22 to 0.27, outperforming AffordMotion (denoted as AM).
% \textbf{(2) Crucial Role of Fine-Grained Geometry Information:}
% In the second stage, leveraging geometry information at varying granularities proves critical. Removing the joint condition drastically reduces performance (\textit{e.g.}, FID and R-score in Tab. 5), demonstrating the importance of fine-grained contact in achieving superior results.
% % In Table 5, we demonstrate that removing the joint condition leads to a drastic reduction in performance, particularly in terms of FID and R-score. This highlights the crucial role that fine-grained contact information plays in enhancing performance.
% \textbf{(3) Textual Information Generation:}
% Furthermore, our pipeline has the potential to generate the textual information, provide the reasoning ability, which is lacking in AM.

% \noindent\textcolor{red}{\textbf{(mWgN)}}
% \reply{\textbf{\uline{Effect of joint loss.}}}
% \textbf{(1) Joint-Level Control:}
% Our pipeline provides the ability to incorporate joint-level control, while AM cannot add joint loss during inference, as its first stage lacks fine-grained information generation. 
% We conducted an experiment by adding a loss function to AM that minimizes the distance between joints and the closest object vertices, but the results remained less effective than ours, as the absence of detailed joint information limits its performance. 
% Additionally, our model outperforms AM on FID, R-score, and diversity by a large margin, even without applying any additional loss.
% \textbf{(2) Balanced Performance:}
% The joint-level loss does contribute to improved contact score, but it may lead to a decrease in FID due to potential distortions. We avoid these issues by incorporating multi-level geometric and semantic information, ensuring that the benefits of fine-grained contact are realized without introducing serious distortions. 
% \begin{table}[h]
% \vspace{-2ex}
% % \caption{Ablation study on joint constraint control (selected metrics).}
% \resizebox{\linewidth}{!}{ 
% \centering
% \begin{tabular}{c|cccccccc}
% \hline
% Method & MPJPE$\downarrow$ & $C_{prec}\uparrow$ & $C_{acc}\uparrow$ & F1$\uparrow$ & FID$\downarrow$ & R-score$\uparrow$ & Div$\uparrow$ & FS$\downarrow$ \\ \hline
% AM                & 25.34   & 0.45   & 0.31 &0.16  & 4.71   & 0.45   & 8.15   & 0.43 \\ \hline
% AM-Loss           & 21.60   & 0.69   & 0.45 &0.36  & 4.13   & 0.47   & 8.25   & 0.65 \\ \hline
% Ours (w/o Loss)   & 22.89   & 0.61   & 0.38 &0.25  & \textbf{0.89}   & \textbf{0.67}   & 10.05  & \textbf{0.38} \\ \hline
% Ours              & \textbf{16.62}   & \textbf{0.84}   & \textbf{0.85} &\textbf{0.77}  & 1.17   & 0.66   & \textbf{10.15}  & 0.57 \\ \hline
% \end{tabular}
% }
% \label{tab:selected_contact}
% \vspace{-3ex}
% \end{table}

% \noindent\textcolor{red}{\textbf{(mWgN,}}
% \textcolor[rgb]{0.55, 0.8, 0.25}{\textbf{jgcn)}}
% \reply{\textbf{\uline{Effectiveness of semantic information.}}} 
% \textbf{(1) Importance of semantic information.}
% Semantic information is beneficial for generating, which provides more context and guides the generation process. Furthermore, our entire pipeline enables reasoning capabilities, allowing for a more comprehensive understanding and generation of human motion.
% \textbf{(2) Experiment of with and w/o semantic information.}
% In the ablation study (Tab. 5), ``no coarse" refers to the absence of semantic information, highlighting the importance of incorporating semantic data into the model, sorry for the misunderstanding.  
% Additionally, we have conducted an experiment on OMOMO with extra semantic information (Supp. Tab. 2), which resulted in a 36\% decrease in FID score, further demonstrating the effectiveness of incorporating semantic information. 
% \textbf{(3) Effectiveness of different level textual information.}
% In the following table, we further clarify the role of different levels of textual information.
% The fine-grained information acts as a supportive element, helping guide the model while also offering the possibility of reasoning about the motion context. 
% \begin{table}[h!]
% % \caption{Ablation study on guidance loss.}
% \vspace{-2ex}
% \resizebox{\linewidth}{!}{ 
% \begin{tabular}{cc|cccccccc}
% \hline
% $Text_{\text{c}}$ & $Text_{\text{f}}$   & MPJPE$\downarrow$ & $C_{prec}\uparrow$ & $C_{acc}\uparrow$ & F1$\uparrow$ & FID$\downarrow$ & R-score$\uparrow$ & Div$\uparrow$  \\ \hline
% & & 24.04 & 0.72 & 0.68 & 0.57 & 1.51 & 0.50 & 9.92
% \\ \hline
% {\checkmark}      &        & \textbf{16.62}    & 0.84               & 0.85              & 0.77         & 1.17            & 0.66              & \textbf{10.15}  %&0.57         
% \\ \hline
%                   & {\checkmark}        & 17.84             & 0.83               & \textbf{0.87}              & 0.77         & 2.24            & 0.45              & 9.90          % & 2.31          
%                   \\ \hline
% {\checkmark}      & {\checkmark}        & 17.01             & \textbf{0.84}      & 0.86     & \textbf{0.77} & \textbf{1.03}   & \textbf{0.68}     & 10.05          & %\textbf{0.46} 
% \\ \hline
% \end{tabular}
% }
% \label{tab:re-text}
% \vspace{-3ex}
% \end{table}

% \noindent\textcolor[rgb]{0.55, 0.8, 0.25}{\textbf{(jgcn)}}
% \reply{\textbf{\uline{Functionality of JointTransformer.}}} 
% The JointTransformer extracts joint features by processing concatenated inputs of text, point cloud, and noisy signals through multi-head self-attention and a feedforward layer. These features interact with affordance information and pass through a linear layer, producing a noise-added joint representation in the diffusion process.

% \noindent\textcolor[rgb]{0.55, 0.8, 0.25}{\textbf{(jgcn)}}
% \reply{\textbf{\uline{Clarity in writing.}}} 
% Regarding the affordance maps (A and A'), we apologize for the confusion. A' refers to the generated affordance map from the first stage, while A represents the ground truth. The variable $x_A$ denotes the affordance map in the diffusion process. We will revise the writing for improved clarity.
% Thanks for pointing this out.
% % \noindent\textcolor[rgb]{0.55, 0.8, 0.25}{\textbf{(jgcn)}}
% % \reply{\textbf{\uline{how semantic and geometric constraints collaborate.}}}

% \noindent\textcolor[rgb]{0.55, 0.8, 0.25}{\textbf{(jgcn)}}
% \reply{\textbf{\uline{Generalizability.}}} 
% In one experiment, we directly sample on HoDome (Tab.4), which features entirely unseen and diverse objects, highlighting the generalizability of our method. We outperform others in this challenging setting. Additionally, we present experiment results on the human-human interaction task in the table below, further demonstrating the adaptability of our model to varied scenarios.

% \noindent\textcolor{blue}{\textbf{(WDaT)}}
% \reply{\textbf{\uline{Comparison with others on human-human interactions.}}} We present a comparison on the human-human interaction (HHI) in the table below. Even compared with RegenNet which is specifically designed for HHI, our method achieves superior results  on most metrics.
% \begin{table}[h]
% \vspace{-2ex}
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{c|cccccccc}
% \hline
% Method     & MPJPE$\downarrow$ & $C_{prec}\uparrow$ & $C_{acc}\uparrow$ & $F1\uparrow$ & FID$\downarrow$ & R-score$\uparrow$ & Div$\uparrow$ & FS$\downarrow$ \\ \hline
% SceneDiff  & 17.18             & 0.70               & 0.54              & 0.52             & 1.81            & 0.23              & 5.88          & 0.49           \\ \hline
% MDM-PC     & 17.19             & 0.72               & 0.58              & 0.56             & \textbf{0.89}   & 0.25              & \textbf{6.27} & 0.38           \\ \hline
% Regennet     &16.14 & 0.79 & 0.58 & 0.60 & 0.73 & 0.25  & 6.01 & 0.48  \\ \hline
% Ours       & \textbf{15.77}    & \textbf{0.83}      & \textbf{0.65}     & \textbf{0.64}    & 1.36            & \textbf{0.29}     & 5.63          & \textbf{0.26}  \\ \hline
% \end{tabular}
% }
% \vspace{-2ex}
% \label{tab:hhi}
% \end{table}

% \noindent\textcolor{blue}{\textbf{(WDaT)}}
% \reply{\textbf{\uline{Speed and real-time performance.}}}
% The current inference process exceeds one second, making it unsuitable for real-time applications. However, diffusion-based generative methods, including those used for comparison in our work, typically take longer due to the nature of diffusion models.
% For entertainment applications scenarios, where real-time performance is not required, and the focus is on achieving sota quality. For these cases, our method prioritizes quality over speed to meet the demands.
% For real-time applications, we acknowledge this as a common challenge and we plan to explore more efficient diffusion methods and consider model
%  distillation to reduce processing time while maintaining high-quality results. Thank you for your valuable suggestion regarding speed.

% \iffalse
% \begin{table*}[h!]
% % \caption{Ablation study on guidance loss.}
% \vspace{-2ex}
% \resizebox{\linewidth}{!}{ 
% \begin{tabular}{c|c|cccccccccccc}
% \hline
% $Text_{\text{c}}$ & $Text_{\text{f}}$   & HandJPE$\downarrow$                                & MPJPE   $\downarrow$                               & $C_{prec} \uparrow$                       & $C_{rec}\uparrow$                       & $C_{acc}\uparrow$ & c\%$\uparrow$    & F1 $\uparrow$   & FID $\downarrow$ & R-score $\uparrow$  & Diversity $\uparrow$ & FS $\downarrow$  \\ \hline
% {\checkmark}          &   & \textbf{27.84}     & \textbf{16.62}    & 0.84               & 0.74               & 0.85                       & 0.66          & 0.77        & 1.17    & 0.66  & \textbf{10.15}       & 0.57   \\\hline
%            & {\checkmark}       &27.85  & 17.84 &     0.83      &   0.75    & 0.87           &0.67&     0.77        &    2.24   &  0.45     &  9.90 & 2.31  \\\hline
% {\checkmark}   &   {\checkmark}    & 27.97              & 17.01             & \textbf{0.84}      & \textbf{0.75}      & \textbf{0.86}      & \textbf{0.67} & \textbf{0.77} & 1.03   &0.68 & 10.05               & \textbf{0.46}  \\\hline 

% \end{tabular}
% }
% \label{tab:loss}
% \vspace{-2ex}
% \end{table*}
% \fi
% % \reply{\textbf{\uline{The effectiveness of fine-grained . }}} 

% %%%%%%%%% BODY TEXT - ENTER YOUR RESPONSE BELOW

% % When placing figures in \LaTeX, it is almost always best to use \verb+\includegraphics+, and to specify the  figure width as a multiple of the line width as in the example below
% % {\small\begin{verbatim}
% %    \usepackage{graphicx} ...
% %    \includegraphics[width=0.8\linewidth]
% %                    {myfile.pdf}
% % \end{verbatim}
% % }


% %%%%%%%%% REFERENCES
% % {
% %     \small
% %     \bibliographystyle{ieeenat_fullname}
% %     \bibliography{main}
% % }

% \end{document}


==> sec/sup_exp.tex <==
\begin{table*}[h!]
\caption{Ablation study on joint constrain control.}
\resizebox{\linewidth}{!}{ 
\centering
\begin{tabular}{c|cccccccccccc}
\rowcolor[HTML]{D9E1F4} 
\hline
joint constrain & HandJPE$\downarrow$                                & MPJPE   $\downarrow$                               & $C_{prec} \uparrow$                       & $C_{rec}\uparrow$                       & $C_{acc}\uparrow$ & c\%$\uparrow$    & F1 $\uparrow$   & FID $\downarrow$ & R-score $\uparrow$   & Diversity $\uparrow$ & FS $\downarrow$  \\ \hline
plevs                        &    52.33        &   26.42    & 0.69           & 0.25           &    0.44          &    0.23 &  0.33  &  14.87   &  0.31  & 7.54 & 0.70  \\ \hline
hand                        &  27.84                           & 16.62                               & 0.84                         & 0.74                            & 0.85       & 0.66    & 0.77 &   1.17  &    0.66     &10.15& 0.57      \\ \hline
random                       &  45.06          &   23.21    &   0.67    &  0.30   & 0.48           &        0.28      &   0.38  & 10.28   &  0.40    & 7.52 & 0.57   \\ \hline
foot                         &   44.89         &   19.29    &  0.62          &     0.22       &       0.41       &   0.21  &  0.30  &  16.75   &   0.32  &  6.87  &  0.59  \\ \hline
\end{tabular}
}
\label{tab:contact}
\end{table*}

